Security Vetting Process of Smart-home Assistant Applications: A First Look and Case Studies

The popularity of smart-home assistant systems such as Amazon Alexa and Google Home leads to a booming third-party application market (over 70,000 applications across the two stores). While existing works have revealed security issues in these systems, it is not well understood how to help application developers to enforce security requirements. In this paper, we perform a preliminary case study to examine the security vetting mechanisms adopted by Amazon Alexa and Google Home app stores. With a focus on the authentication mechanisms between Alexa/Google cloud and third-party application servers (i.e. endpoints), we show the current security vetting is insufficient as developer mistakes can not be effectively detected and notified. A weak authentication would allow attackers to spoof the cloud to insert/retrieve data into/from the application endpoints. We validate the attack through ethical proof-of-concept experiments. To confirm vulnerable applications have indeed passed the security vetting and entered the markets, we develop a heuristic-based searching method. We find 219 real-world Alexa endpoints that carry the vulnerability, many of which are related to critical applications that control smart home devices and electronic cars. We have notified Amazon and Google about our findings and offered our suggestions to mitigate the issue.

==> conclusion.tex <==
\section{Conclusion}
In this paper, we systematically investigate the authentication mechanism between the Alexa/Google cloud and third-party endpoints.
We find that both Alexa and Google did not carefully enforce an authentication mechanism, which allows vulnerable skills to enter the application stores. Through proof-of-concept attacks and empirical measurements, we demonstrate the feasibility of spoofing the cloud and performing SQL injection attacks on vulnerable endpoints. We also discover vulnerable endpoints of real-world skills. Our results provide new insights into the security of the backend services for smart-home assistant systems. 
